Holi-Spatial: Evolving Video Streams into Holistic 3D Spatial Intelligence

The pursuit of spatial intelligence fundamentally relies on access to large-scale, fine-grained 3D data. However, existing approaches predominantly construct spatial understanding benchmarks by generating question-answer (QA) pairs from a limited number of manually annotated datasets, rather than systematically annotating new large-scale 3D scenes from raw web data. As a result, their scalability is severely constrained, and model performance is further hindered by domain gaps inherent in these narrowly curated datasets. In this work, we propose Holi-Spatial, the first fully automated, large-scale, spatially-aware multimodal dataset, constructed from raw video inputs without human intervention, using the proposed data curation pipeline. Holi-Spatial supports multi-level spatial supervision, ranging from geometrically accurate 3D Gaussian Splatting (3DGS) reconstructions with rendered depth maps to object-level and relational semantic annotations, together with corresponding spatial Question-Answer (QA) pairs. Following a principled and systematic pipeline, we further construct Holi-Spatial-4M, the first large-scale, high-quality 3D semantic dataset, containing 12K optimized 3DGS scenes, 1.3M 2D masks, 320K 3D bounding boxes, 320K instance captions, 1.2M 3D grounding instances, and 1.2M spatial QA pairs spanning diverse geometric, relational, and semantic reasoning tasks. Holi-Spatial demonstrates exceptional performance in data curation quality, significantly outperforming existing feed-forward and per-scene optimized methods on datasets such as ScanNet, ScanNet++, and DL3DV. Furthermore, fine-tuning Vision-Language Models (VLMs) on spatial reasoning tasks using this dataset has also led to substantial improvements in model performance.

==> tables/02_eval_on_mindcube.tex <==
    
    
    
    
    


\begin{table}[tbp]
\centering
\caption{Left: \name data statistics. The number next to the setting (\textsc{Rotation}, \textsc{Among}, \textsc{Around}) means the total QA pairs. Numbers next to each dataset (e.g., Arkitscenes) mean QA pairs/image groups. For example, ``865/53'' for Arkitscenes in \textsc{Rotation} means we have 865 QA pairs and 53 image groups from it. Right: Performance of VLMs on \name.  \textcolor{black}{\colorbox{blue!7}{Dark blue}} indicates the best result among all models and \textcolor{black}{\colorbox{blue!4}{light blue}} indicates the best result among open-source models.} \label{tab:mindcube_stats_eval_results}
\vspace{0.5em}
\begin{minipage}{0.27\textwidth}
\centering

    \includegraphics[width=\textwidth]{figs/statistics.pdf} 

\end{minipage}
\hfill
\begin{minipage}{0.68\textwidth}
\centering
\resizebox{\linewidth}{!}{%
  \begin{tabular}{lcccccc}
 \textbf{Method}      & \cellcolor[HTML]{E8E8E8} \textbf{Overall}  & \cellcolor[HTML]{CFDDA6} \textbf{Rotation} & \cellcolor[HTML]{DABFDA} \textbf{Among} & \cellcolor[HTML]{FDEEC7} \textbf{Around} \\
    \hline
\rowcolor{tableblue}
\textit{Baseline} &&&&\\
  \it \textcolor{gray}{Random (chance)} & \it \textcolor{gray}{32.35}  & \it \textcolor{gray}{36.36} & \it \textcolor{gray}{32.29} & \it \textcolor{gray}{30.66} \\
     \it \textcolor{gray}{Random (frequency)} & \it \textcolor{gray}{33.02}  & \it \textcolor{gray}{38.30} & \it \textcolor{gray}{32.66} & \it \textcolor{gray}{35.79} \\
    \hline
\rowcolor{tableblue}
\textit{Open-Weight Multi Image Models} & \rule{0pt}{1em} & \rule{0pt}{1em} & \rule{0pt}{1em} & \rule{0pt}{1em} \\
     LLaVA-Onevision-7B~\cite{onevision}     &  \cellcolor{blue!4}47.43  & 36.45 & \cellcolor{blue!4}48.42 & 44.09 \\
     LLaVA-Video-Qwen-7B~\cite{llava-video}   &  41.96  & 35.71 & 43.55 & 30.12 \\
     LongVA-7B~\cite{longva}     & 29.46  &  35.89 & 29.55 & 24.88 \\
     mPLUG-Owl3-7B-241101~\cite{mplug-owl3}   & 44.85  & 37.84 & 47.11 & 26.91  \\
     InternVL2.5-8B~\cite{chen2024internvl}        & 18.68  & 36.45 & 18.20 & 13.11 \\
     Qwen2.5-VL-7B-Instruct~\cite{Qwen2.5-VL}         & 29.26  & \cellcolor{blue!4}38.76 & 29.50 & 21.35  \\
     Qwen2.5-VL-3B-Instruct~\cite{Qwen2.5-VL}         & 33.21  & 37.37 & 33.26 & 30.34  \\
     Idefics-8B-Llama3~\cite{laurenccon2024building}     & 35.86  & 35.15 & 35.94 & 35.49 \\
     DeepSeek-VL2-Small~\cite{lu2024deepseekvlrealworldvisionlanguageunderstanding}    &  \cellcolor{blue!7}47.62  & 37.00 & \cellcolor{blue!7}50.38 & 26.91 \\

     Gemma-3-12B-it~\cite{team2025gemma} & 46.67 & 38.39 & 48.38 & 34.63\\
     Mantis-8B (SigLip)~\cite{mantis} &  41.05 & 37.65 & 40.23 & \cellcolor{blue!7}50.99  \\
    \hline
    
    
\rowcolor{tableblue}
\textit{Proprietary Models} & \rule{0pt}{1em} & \rule{0pt}{1em} & \rule{0pt}{1em} & \rule{0pt}{1em} \\
     GPT-4o~\cite{gpt4o_blog}  &  38.81 & 32.65 & 40.17 & 29.16 \\
     Claude-4-Sonnet-20250514~\cite{anthropic_claude4_2025}    &  44.75  & \cellcolor{blue!7}48.42 & 44.21 & \cellcolor{blue!4}47.62 \\
    \hline
    
\rowcolor{tableblue}
\textit{Spatial Models}&&&& \\
     RoboBrain~\cite{ji2025robobrain} & 37.38 & 35.80 & 38.28 & 29.53 \\
     SpaceMantis~\cite{space-mantis}    & 22.81  & 37.65 & 21.26 & 29.32 \\ 
     Spatial-MLLM~\cite{wu2025spatial} & 32.06 & 38.39 & 20.92 & 32.82 \\
     Space-Qwen~\cite{space-mantis}    & 33.28  & 38.02 & 33.71 & 26.32 \\
  \end{tabular}
 }
\end{minipage}

\vspace*{-1em}
\end{table}

